All Languages Matter: Evaluating LMMs on Culturally Diverse 100 Languages

Existing Large Multimodal Models (LMMs) generally focus on only a few regions and languages. As LMMs continue to improve, it is increasingly important to ensure they understand cultural contexts, respect local sensitivities, and support low-resource languages, all while effectively integrating corresponding visual cues. In pursuit of culturally diverse global multimodal models, our proposed All Languages Matter Benchmark (ALM-bench) represents the largest and most comprehensive effort to date for evaluating LMMs across 100 languages. ALM-bench challenges existing models by testing their ability to understand and reason about culturally diverse images paired with text in various languages, including many low-resource languages traditionally underrepresented in LMM research. The benchmark offers a robust and nuanced evaluation framework featuring various question formats, including true/false, multiple choice, and open-ended questions, which are further divided into short and long-answer categories. ALM-bench design ensures a comprehensive assessment of a model's ability to handle varied levels of difficulty in visual and linguistic reasoning. To capture the rich tapestry of global cultures, ALM-bench carefully curates content from 13 distinct cultural aspects, ranging from traditions and rituals to famous personalities and celebrations. Through this, ALM-bench not only provides a rigorous testing ground for state-of-the-art open and closed-source LMMs but also highlights the importance of cultural and linguistic inclusivity, encouraging the development of models that can serve diverse global populations effectively. Our benchmark is publicly available.

==> Tables/AnnotationErrors.tex <==
% Semantic error (meaning completely ruined in the translation)
% Cultural error (use of correct but unusual words not used by locals in day-to-day language)
% Contextual error (use of words that doesn’t match context, ex: The statue is living in Hawaii instead of The statue is located in Hawaii)
% Language error (when translation is given in characters of a different alphabet)
% Grammatical error (meaning is correct but just some grammar-related errors are present, if the true meaning of the sentence is not grasped in the translation along with grammar errors, please refer it as "Semantic error”)

\begin{table}[!htp]
\centering
% \vspace{-0.2in}
\resizebox{0.2\textwidth}{!}{
\begin{tabular}{@{}l@{}}
\toprule
\textbf{Mistake Category} \\ \midrule
1. Semantic Error \\ 
2. Cultural Error \\ 
3. Contextual Error \\ 
4. Language Error \\ 
5. Grammatical Error \\ \bottomrule
\end{tabular}
}
\caption{Types of Mistakes in the translations.}
\vspace{-0.1in}
\label{tab:Annotation Guidelines}
\end{table}

==> Tables/Data_Stats.tex <==
\begin{table}[!htp]
\centering
% \vspace{-0.2in}
\resizebox{0.35\textwidth}{!}{
\begin{tabular}{lr}
\toprule
\textbf{Category} \\ \midrule
No. of Images & 5,151 \\
No. of Questions & 22,870 \\
No. of Countries & 73 \\
No. of Languages & 100 \\
No. of Categories & 13 \\
No. of Language Scripts & 11 \\
Total Multiple Choice & 5628 \\
Total True/False & 2807 \\
Total Short Questions & 6828 \\
Total Long Questions & 7607 \\
% No. of Country-Language pairs & 33 \\
Avg. Questions per Image &  4.43 \\
Avg. Words per Question & 12.05 \\
Avg. Words per Answer & 42.65 \\ \bottomrule
\end{tabular}
}
\caption{ALM Data Statistics}
\vspace{-0.1in}
\label{table:data_statistics}
\end{table}

==> Tables/ablations.tex <==
\begin{table}[!htp]
    \centering
    \setlength{\tabcolsep}{4pt}
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{lccccccccccccc}
        \toprule
        \textbf{Image Source} & \multicolumn{2}{c}{\textbf{LLaVA-1.5-7B}} & \multicolumn{2}{c}{\textbf{M-CLIP}} & \multicolumn{2}{c}{\textbf{CLIP}} & \multicolumn{2}{c}{\textbf{mBLIP-mT0}} & \multicolumn{2}{c}{\textbf{mBLIP-BLOOMZ}} & \multicolumn{2}{c}{\textbf{InstructBLIP}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
        & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} \\
        \midrule
        Few-Shot Method  & 47.0 & 34.0 & 37.9 & 34.0 & 41.5 & 30.4 & 34.4 & 31.9 & 40.5 & 34.2 & \textbf{49.1} & \underline{31.1} \\
        English-Translation Eval  & \textbf{48.0} & \underline{37.0} & 36.8 & 33.6 & 44.1 & 33.1 & 34.0 & 32.8 & 39.6 & 33.5 & 46.7 & 33.1 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Ablation table, row 1 will show a few-shot example. Row 2 will show evaluating in English, translation in the local language and then evaluating with GPT.}
    \label{tab:image_source_accuracy}
\end{table}

==> Tables/results_across_categories.tex <==
\begin{table}[!htp]
    \centering
    \setlength{\tabcolsep}{4pt}
    \resizebox{0.50\textwidth}{!}{%
    \begin{tabular}{lccccccccccccc}
        \toprule
        \textbf{Categories} & \multicolumn{2}{c}{\textbf{LLaVA-1.5-7B}} & \multicolumn{2}{c}{\textbf{M-CLIP}} & \multicolumn{2}{c}{\textbf{CLIP}} & \multicolumn{2}{c}{\textbf{mBLIP-mT0}} & \multicolumn{2}{c}{\textbf{mBLIP-BLOOMZ}} & \multicolumn{2}{c}{\textbf{InstructBLIP}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
        & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} & \textbf{EN} & \textbf{LOC} \\
        \midrule
        Brands          & \textbf{47.7} & \underline{36.5} & 37.8 & 35.4 & 40.1 & 31.3 & 33.5 & 31.3 & 40.3 & 36.5 & 46.9 & 32.2 \\
        Food            & \textbf{45.9} & \underline{32.5} & 33.1 & 29.1 & 40.8 & 30.9 & 27.8 & 26.9 & 37.4 & 30.7 & 43.8 & 32.0 \\
        Geography       & \textbf{46.1} & \underline{37.9} & 36.5 & 35.6 & 41.0 & 32.7 & 31.1 & 32.6 & 35.1 & 32.6 & 43.6 & 32.5 \\
        Objects         & 50.5 & 34.7 & 36.4 & 32.7 & 39.0 & 26.4 & 33.4 & 31.6 & \textbf{52.0} & \underline{43.2} & 42.8 & 31.6 \\
        People          & \textbf{58.6} & \underline{38.7} & 45.7 & 38.2 & 44.9 & 36.4 & 34.4 & 34.1 & 47.1 & 37.6 & 58.3 & 38.1 \\
        Plants \& Animals & 54.8 & 39.4 & 40.6 & 31.9 & 45.9 & 27.9 & 35.4 & 35.9 & 46.4 & 33.0 & \textbf{56.8} & \underline{34.8} \\
        Pop Culture     & \textbf{43.5} & \underline{36.7} & 32.6 & 31.6 & 44.5 & \underline{37.1} & 30.7 & 35.8 & 37.0 & 30.7 & 45.0 & 35.5 \\
        Sports          & \textbf{52.0} & 40.0 & 40.2 & 32.6 & 45.7 & 34.6 & 33.9 & 31.3 & 49.7 & 36.4 & 46.5 & \underline{37.5} \\
        Tradition       & \textbf{48.8} & \underline{37.1} & 36.6 & 34.9 & 39.4 & 30.9 & 32.9 & 32.9 & 46.0 & 32.9 & 46.5 & 30.7 \\
        Vehicles        & \textbf{50.9} & 43.8 & 38.4 & 39.4 & 40.5 & 32.6 & 37.4 & 35.7 & 42.1 & 33.3 & \textbf{52.6} & \underline{33.3} \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Accuracy of models across categories. Per category, the best-performing models on English (EN) and local language (LOC) question-option pairs are bolded and underlined, respectively.}
    \label{tab:model_accuracy}
\end{table}

